Deep Bayesian Active Learning for Accelerating Stochastic Simulation

Stochastic simulations such as large-scale, spatiotemporal, age-structured epidemic models are computationally expensive at fine-grained resolution. While deep surrogate models can speed up the simulations, doing so for stochastic simulations and with active learning approaches is an underexplored area. We propose Interactive Neural Process (INP), a deep Bayesian active learning framework for learning deep surrogate models to accelerate stochastic simulations. INP consists of two components, a spatiotemporal surrogate model built upon Neural Process (NP) family and an acquisition function for active learning. For surrogate modeling, we develop Spatiotemporal Neural Process (STNP) to mimic the simulator dynamics. For active learning, we propose a novel acquisition function, Latent Information Gain (LIG), calculated in the latent space of NP based models. We perform a theoretical analysis and demonstrate that LIG reduces sample complexity compared with random sampling in high dimensions. We also conduct empirical studies on three complex spatiotemporal simulators for reaction diffusion, heat flow, and infectious disease. The results demonstrate that STNP outperforms the baselines in the offline learning setting and LIG achieves the state-of-the-art for Bayesian active learning.

==> sections/exp_old.tex <==


% \mc{We probably need a short introduction paragraph here to describe the role of the experiments.}
We start with a simple susceptible-exposed-infectious-removed (SEIR) compartmental model. We compare our method with Gaussian process  for validation. We then apply our \ours{} framework to mimic the dynamics of a real-world large-scale Local Epidemic and Mobility model (LEAM-US) simulator and report the performance using different acquisition functions. We implement GP using {gpytorch}  \citep{gardner2018gpytorch}  with Matern kernel. All NP models are implemented using pytorch \citep{paszke2019pytorch}.


\subsection{SEIR Compartmental Model}

\textbf{SEIR Simulation.}
To show that \ours{} indeed provides a more flexible and faster alternative to GP, we begin with a simple stochastic, discrete, chain-binomial SEIR compartmental model as our stochastic simulator. In this model,  susceptible individuals ($S$) become exposed ($E$) through interactions with infectious individuals ($I$), details of the model are deferred to the Appendix \ref{app:seir_model}.



We set the total population  $N=S+E+I+R$ as $100,000$, the initial number of exposed individuals as $E_0=2,000$, and the initial number of infectious individuals as $I_0=2,000$. The latent period varies between approximately $1.5$ to $4$ days, i.e. latent individuals move to the infectious stage at a rate $\varepsilon \in [0.25,0.65]$ (step 0.05) that is inversely proportional to the latent period, the infectious period $\mu^{-1}$ is set to be equal to 1 day,  and we let the basic reproduction number $R_0$ (which in this case coincides with the transmissibility rate $\beta$) vary between $1.1$ and $4.0$ (step $0.1$). Here, each $(\beta,\varepsilon)$ pair corresponds to a specific scenario, which determines the parameters $\theta$. We simulate the first $100$ days of the epidemic with a total of $300$ scenarios and generate $30$ samples for each scenario.
%Since $\mu$ is fixed at 1, The value of $\beta$ is the same as the reproduction number $R0$. We set the search space of $\beta$ from 1.1 to 4 with 0.05 interval. For each scenario, we run SEIR simulator 50 times to generate the samples.


\textbf{Model Implementation.}
We compare \ours{}  with GP for Bayesian active learning.  In this toy experiment, we only predict the number of individuals in the infectious compartment. The input is $(\beta,\varepsilon)$ pair and the output is the $100$ days' infection prediction. As the simulator is simple, we use the vanilla NP model with the global latent variable $z$ (Fig. \ref{fig:graphical_model} NP).
% As the simulator is simple, our NP model only has two fully-connected layers for the encoder and the  decoder.
For each epoch, we randomly select $10\%$  of the samples as context.  Implementation details are deferred to Appendix \ref{app:implementation}.

%  The dimension of latent vector $z$ is set at 4. We use Adam optimizer with early stopping.   We trained GP model for $300$ steps with learning rate fixed at $10^{-1}$.  The learning rate is fixed at $10^{-3}$.
%

% For NP, the input includes a fixed $R_{0}$ sequence with length at 51 together with the three fixed initial compartments. The output is the same as GP. The NP model uses two fully-connected layers for the encoder and the  decoder. The dimension of latent vector $z$ is set at 4. We use Adam optimizer and use early stopping with patience fixed at 1000 epoch. The learning rate is fixed at $10^{-3}$. For each epoch, it randomly selects $25\%$ samples as context. The model is implemented by pytorch \cite{paszke2019pytorch}. 

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.47\linewidth,trim={20 20 20 20}]{iclr_figs/seir_npgp_pred.pdf}
%   \includegraphics[width=0.47\linewidth,trim={20 20 20 20}]{iclr_figs/seir_npgp_ac_comp.pdf}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{10cm}{0cm}}
%   \caption{Neural Processes vs. Gaussian Processes for Bayesian active learning in SEIR compartmental model. Left: uncertainty quantification comparison with the truth. Right: MAE loss versus the percentage of data for both NP and GP using different acquisition functions.}
%   \label{fig:npvsgp}
% \end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{iclr_figs/fig3.pdf}
  \caption{Neural Processes vs. Gaussian Processes for Bayesian active learning in SEIR compartmental model. Left: uncertainty quantification comparison with the truth. Right: MAE loss versus the percentage of data for both NP and GP using different acquisition functions.}
  \label{fig:npvsgp}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{iclr_figs/fig4.pdf}
    \caption{NP Acquisition functions behavior visualization in 2D. For each iteration, top row represents the current MAE mesh in infectious population for all $(\beta,\varepsilon)$ candidates.
    % For each iteration, top row represents the current test MAE in infectious population.
    Bottom row is the score evaluated by the acquisition function. Yellow dots are existing parameters. Red stars are the newly selected parameters. }
    \label{fig:seir_acq_visual}
\end{figure}

%
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.7\linewidth,trim={20 20 20 20}]{figs/seir_mae_loss.pdf}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{10cm}{0cm}}
%   \caption{MAE loss versus number of examples for both NP and GP using SEIR simulator.}
%   \label{fig:seir_mae}
% \end{figure}
% Both models are fitted by the same $11$ observations selected randomly.

\textbf{Uncertainty Quantification.}
Figure \ref{fig:npvsgp} compares the NP and GP performance on one scenario in the held-out test set. It shows  the ground truth and the predicted number of infectious population for the first $50$ days. We also include the confidence intervals (CI) with $5$ standard deviations for ground truth and NP predictions and $1$ standard deviation for GP predictions. We observe that NP fits the simulation dynamics better than GP for mean prediction. Moreover, NP has closer CIs to the truth, reflecting  the simulator's intrinsic uncertainty.  GP shows larger CIs which represent the model's own uncertainty. Note that NP is much more flexible than GP and can scale easily to high-dimensional data.
% Note that the black star in Figure \ref{fig:npvsgp} represents the $R0$ scenario already selected. The truth on the y axis is the average values for  50 samples for each $R0$. Therefore, the confidence interval of both NP and GP will not be too narrow for the observed $R_{0}$.

\textbf{Acquisition Functions.}  
We  compare different acquisition functions in Bayesian active learning. We  select 2  scenarios as the initial training dataset. Then we continue augmenting the training set using the remaining scenarios until the validation loss converges. GP is not a latent variable model, hence LIG does not apply.  We report the average test  mean absolute error (MAE) over three random runs. The candidate set for training includes $270$ scenarios. We set aside $15$ scenarios each for validation and test. The scenarios are evenly distributed in the search space.

% For GP and NP, we use Mean STD and Maximum Entropy as two acquisition functions and compare them with random sampling as baseline. We also include MaxZdiff for NP. 


% Mean STD is the best, which only requires $16.9\%$ of the training samples to converge, while Maximum Entropy takes $22\%$ and random sampling takes $28.8\%$ to converge. , while random sampling takes $28.8\%$ and Maximum Entropy takes $40.7\%$ of samples to converge.

Figure \ref{fig:npvsgp} shows the testing MAE over percentage of data used for training for NP and GP with different acquisition functions. None of the GP methods converge after selecting $4.07\%$ of the data for training while NP methods converge much faster. Our proposed acquisition function LIG is more sample efficient in NP. It   takes only $4.07\%$ of the data to converge and reach the NP offline performance, which uses the entire training set for training. This validates our theory that the uncertainty of the deep surrogate model is better measured on the latent space instead of the predictions.

% Figure \ref{fig:npvsgp} shows that random sampling converges similarly for  NP and GP. Mean STD and Maximum Entropy are more sample efficient in GP, with Mean STD being $41.3\%$ more sample efficient than random sampling. However, on neural processes, both methods are worse than random sampling   while our proposed method LIG excels. This also validates our theory that the uncertainty of the deep surrogate model is better measured on the latent space instead of the predictions.  LIG takes only $16.9\%$ of samples to converge, which is as efficient as Mean STD on GP. Mean STD fails to converge after using $49.2\%$ of the samples. 

\textbf{Exploration Exploitation Trade-off.} To understand the large performance gap for  LIG vs. baselines on NP, we visualize the values of test MAE and the reward from acquisition functions for each Bayesian active learning iteration, shown in Figure \ref{fig:seir_acq_visual}.  For Mean STD and Maximum Entropy, both tend to exploit the region with large transmission rate for the first $2$ iterations. Including these scenarios makes the training set unbalanced. The MAE in the region with small transmission rate become worse after $2$ iterations. Meanwhile, Random  is doing pure exploration. The improvement of MAE performance is not apparent after $2$ iterations. Our proposed LIG 
is able to reach a balance by exploiting the uncertainty in the latent process and encouraging exploration. Hence, with a small number of iterations ($I=2$), it has already selected ``informative scenarios'' in the search space.

% \textbf{Exploration Exploitation Trade-off.} To understand why there is a large performance gap for  MaxEntropy and Mean STD on GP vs. NP, we visualize the predictions for each Bayesian active learning iteration, shown in Figure \ref{fig:seir_acq_visual}.  For GP, both Mean STD and MaxEntropy depend on the model's predictive uncertainty. \ryu{rewrite} Hence, with a small number of iterations ($I=7$), they have already selected the scenarios including important information of the search space. However, For NP, its uncertainty reflects the intrinsic uncertainty of the simulator, rather than the NP model itself. Using predictive uncertainty tends to be  over-conservative and  without much exploration. LIG solves this problem by exploiting the uncertainty in the latent process and encouraging exploration.  Its active learning behavior is  similar to what Mean STD selected on GP. 


% For Bayesian active learning part, we first add samples from three scenarios with different $R0$ selected randomly to the training set, and then select one scenario from the remained search space for each iteration based on the acquisition functions and add its corresponding samples to the training set until the test loss converge. Here, we calculate the test loss using mean absolute error (MAE). The test set includes $59$ different scenarios in the search space. Figure \ref{fig:seir_mae} shows that Bayesian active learning using both MeanSTD and MaxEntropy can help select the scenario from the search space efficiently.





% The game is a two-dimensional grid or lattice consisting of cells. Each cell assumes one of a finite number of
% states at any point in time. A set of simple rules determines
% the value of each cell based on the cell’s previous state.
% Every cell is updated each period according to the rules.
% The next value of a cell depends on the cell’s current value
% and the values of its immediate neighbors in the eight surrounding cells. Each cell is identical in terms of its update
% rules. A CA is deterministic in that the same state for a cell
% and its neighbors always results in the same updated state.
% The GOL has three rules that determine the next state (either On or Off) of each cell:
% \begin{itemize}
%     \item The cell will be On in the next generation if exactly three of its eight neighboring cells are currently On \ry{Allen change the rules}.
%     \item The cell will retain its current state if exactly two
% of its neighbors are On.
% \item  The cell will be Off otherwise. 
% \end{itemize}


\subsection{Local Epidemic and Mobility model (LEAM-US)} \label{covid_deepgleam}

As a real-world experiment, we use a large-scale, spatiotemporal, age-structured epidemic model, LEAM-US, as our stochastic simulator. Our goal is to use \ours{} to mimic the internal mechanism of this simulator to accelerate disease modeling and scenario creation.


\textbf{LEAM-US Simulator.} 
The Local Epidemic and Mobility model (LEAM-US) is a stochastic, spatial, age-structured epidemic model based on a metapopulation approach which divides the US in more than 3,100 subpopulations, each one corresponding to a each US county or statistically equivalent entity.  Population size and county-specific age distributions reflect Census' annual resident population estimates for year 2019. %(\todo{https://www.census.gov/data/datasets/time-series/demo/popest/2010s-counties-total.html }).
%
We consider individuals divided into $10$ age groups. Contact mixing patterns are age-dependent and state specific and modeled considering contact matrices that describe the interaction of individuals in different social settings \citep{mistry2020inferring}.
LEAM-US integrates a human mobility layer, represented as a network, using both short-range (i.e., commuting) and long-range (i.e., flights) mobility data, see more details in Appendix \ref{app:leam_model}. 

%[0-9, 10-19, 20-24, 25-29, 30-39, 40-49, 50-59, 60-69, 70-79, 80+] , namely: households, schools, workplaces, and contacts occurring in the general community

\begin{comment}

Commuting flows between counties are obtained from the 2011-2015 5-Year ACS Commuting Flows survey and properly adjusted to account for differences in population totals since the creation of the dataset. Instead, long-range air traveling flows are quantified using origin-destination daily passenger flows between airport pairs as reported by the Official Aviation Guide (OAG) and IATA databases (updated in 2021) \cite{OAG,IATA}. In addition, flight probabilities are age and country specific.

\textbf{Experiment Setup.} 
Our simulation model is initialized using a multi-scale modeling approach that utilizes GLEAM, the Global and Epidemic Mobility model \cite{balcan2009multiscale,balcan2010modeling,tizzoni2012real,zhang2017spread,chinazzi2020effect,davis2020estimating}, to simulate a set of 500 different initial conditions for LEAM-US starting on February 16th, 2020. The disease dynamics are modeled using a classic SEIR-like model as in the first experiment and the time interval considered for the simulations is February 2020 until December 2020. However, in this second model, travel restrictions, mobility reductions, and government interventions are explicitly modeled to mimic the real timeline of interventions of the events that occurred during the COVID-19 pandemic. Specifically, Google's COVID-19 Community Mobility Reports \cite{google_data} are used to quantify mobility and contact reductions, while non-pharmaceutical interventions and other policy interventions are tracked using the Oxford Covid-19 Government Response Tracker (OxCGRT) \cite{Oxford}. 
\end{comment}

% and it is calibrated to realistically describe the evolution of the COVID-19 pandemic. In particular, LEAM-US is stochastic and produces an ensemble of possible epidemic outcomes for each set of initial conditions. %To account for the potentially different reporting levels of the states, a free parameter Infection Fatality Rate (IFR) multiplier is added to each model. To calibrate and select the most reasonable outcomes, we filter the models by the latest hospitalization trends and confirmed cases trends, and then we select and weight the filtered models using Akaike Information Criterion \citep{zhang2017forecasting}. The forecast of the evolution of the epidemic is formed by the final ensemble of the selected models.

%the world is divided into over 3,200 geographic subpopulations constructed using a Voronoi tessellation of the Earth's surface. Subpopulations are centered around major transportation hubs (e.g. airports) and consist of cells with a resolution of approximately 25 x 25 kilometers \cite{balcan2009multiscale,balcan2010modeling,tizzoni2012real,zhang2017spread,chinazzi2020effect,davis2020estimating}. High resolution data are used to define the population of each cell. Other attributes of individual subpopulations, such as age-specific contact patterns, health infrastructure, etc., are added according to available data \citep{mistry2020inferring}.

%GLEAM integrates a human mobility layer - represented as a network - that uses both short-range (i.e. commuting) and long-range (i.e. flights) mobility data from the Offices of Statistics for $30$ countries on $5$ continents as well as the Official Aviation Guide (OAG) and IATA databases (updated in $2020$). The air travel network consists of the daily passenger flows between airport pairs (origin and destination) worldwide mapped to the corresponding subpopulations. Where information is not available, the short-range mobility layer is generated synthetically by relying on the “gravity law”  or the more recent “radiation law”  both calibrated using real data \citep{Simini2012}. 

%The model is calibrated to realistically describe the evolution of the COVID-19 pandemic as detailed in \cite{chinazzi2020effect,davis2020estimating}.
%Lastly, GLEAM is stochastic and produces an ensemble of possible epidemic outcomes for each set of initial conditions. To account for the potentially different reporting levels of the states, a free parameter Infection Fatality Rate (IFR) multiplier is added to each model. To calibrate and select the most reasonable outcomes, we filter the models by the latest hospitalization trends and confirmed cases trends, and then we select and weight the filtered models using Akaike Information Criterion \citep{zhang2017forecasting}. The forecast of the evolution of the epidemic is formed by the final ensemble of the selected models.
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.47\linewidth,trim={20 70 20 0}]{iclr_figs/leam_stnp_pred.pdf}
%     \includegraphics[width=0.47\linewidth,trim={20 20 20 20}]{iclr_figs/lean_ac_comp.pdf}
%   \caption{Left: \ours{} predictions for the number of individuals in Infectious and Removed compartments in LEAM-US model. Right: acquisition function comparisons on the LEAM-US simulator. MAE loss versus the percentage of samples for \ours{} during Bayesian active learning.}
%   \label{fig:gleam_pred}
% \end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{iclr_figs/fig5.pdf}
  \caption{Left: \ours{} predictions for the number of individuals in Infectious and Removed compartments in LEAM-US model. Right: acquisition function comparisons on the LEAM-US simulator. MAE loss versus the percentage of samples for \ours{} during Bayesian active learning.}
  \label{fig:gleam_pred}
\end{figure}


\textbf{Dataset.}
We separate data in California monthly to predict the 28 days' sequence from the 2nd to the 29th day of each month from March to December. Each $\theta$ includes the county-level parameters of LEAM-US and state level incidence and prevalence compartments. The total number of dimension in $\theta$ is $16,912$, see details in Appendix \ref{app:leam_model}.   Overall, there are $315$ scenarios in the search space, corresponding to $315$ different $\theta$ with total $16,254$ samples. We split $78\%$ of the data as the candidate train set, and $11\%$ for validation and test. We use $8.6\%$ data  for initial training. We first perform offline learning to show that the STNP model can accurately learn the LEAM-US dynamics. For Bayesian active learning, we use the candidate train set as the search space.
% \textbf{Dataset.}
% There are $45$ different scenarios for each month. We separate data monthly to predict the 28 days' sequence from the 2nd to the 29th day of each month from March to December. $78\%$ of the data for candidate set, $11\%$ for validation and test. We use data 11from March to November as training set and divide the December data into two halves for testing and validation \ryu{change}. We first perform offline learning to show that the STNP model can learn the dynamics of LEAM-US. For Bayesian active learning, we use the training dataset as the search space. There are 45 different scenarios for each month. Overall, there are 360 scenarios in the search space, corresponding to 360 different $\theta$ with $18576$ samples.




\textbf{Model Implementation.} We instantiate a STNP model to mimic an epidemic simulator that has $\theta$ at both county and state level and $x_t$ at the state level. We use county-level parameter $\theta$ together with a county-to-county mobility graph $A$ in California as input.  We use the DCGRU layer \citep{li2017diffusion} to encode the mobility graph in a GRU. We use a linear layer to map the county-level output to hidden features  at the state level. For both the state-level encoder and  decoder, we use multi-layer GRUs.     For each epoch, we randomly select $20\%$ samples as  context sequence.

\textbf{STNP Predictions.}
Figure \ref{fig:gleam_pred} left visualize the STNP predictions in four key compartments of a typical scenario with $R_{0}=3.1$ from March 2nd to March 29th. The confidence interval is plotted with $2$ standard deviations. We can see that  both the mean and confidence interval of STNP predictions match the truth well. These results demonstrate the promise that the  generative STNP model can serve as a deep surrogate model for the LEAM-US simulator.

% \paragraph{Accuracy-Computation Trade-off}

\textbf{Acquisition Functions.}
We compare different acquisition functions with STNP. All methods start with the same initial train set. Then we continue adding 8 scenarios to the training set until the validation loss converges. We  measure the average performance over three random runs and report the test MAE.
%
% We compare  different acquisition functions in STNP. The initial training dataset has  8 scenarios from March to November with the same randomly selected $R_{0}$. Then we continue adding 16 scenarios to the training set until the validation loss converges. We use Mean STD, Maximum Entropy, LIG, the combined method with random sampling for the first two iterations plus LIG for the rest of the iterations, and compare them with random sampling as baseline. We  measure the average performance over three random runs and report the test MAE  on  $360$  scenarios.
%
Figure \ref{fig:gleam_pred} right shows the log scale MAE versus the percentage of samples included for training, which is  scales linearly in computation. It shows our proposed LIG always has the best MAE performance until the convergence. Moreover, after using $31.4\%$ of data from the candidate train set, LIG already outperforms the offline model. 

% The right side of Figure \ref{fig:gleam_pred} shows the log scale MAE versus the percentage of samples included for training, which is linear associated with the computation power. Both LIG and the combined method take  $37.7\%$ of the samples to converge, while Mean STD takes $42.2\%$ to converge. Both random sampling and Maximum Entropy take $51.1\%$ to converge. 

% We notice that random sampling with more exploration in the early iterations has a slight advantange. Therefore, we  also  combine the two acquisition functions, leading to the hybrid method Random-LIG. From the figure, we can see that this hybrid method is optimal during the entire learning process until  convergence.
\begin{wraptable}{r}{0.5\linewidth}
\centering
\caption{NP model comparison in LEAM simulator (population divided by 1000) and Reaction-Diffusion simulator.}
\begin{tabular}{c|c|c}
\toprule
Model & MAE (LEAM) & MAE (RD) \\
% ====================== LA ======================
\midrule
NP & 24.2 $\pm$ 5.9 & 3.37 $\pm$ 0.18\\
 \midrule
SNP & 21.8 $\pm$ 0.8 & 3.11 $\pm$ 0.07 \\
 \midrule 
STNP & \textbf{6.3}$\pm$ 0.8 & \textbf{2.84} $\pm$ 0.17\\
\bottomrule
\end{tabular}
\label{tb:offline}
\end{wraptable}

% \begin{wraptable}{r}{0.5\linewidth}
% \centering
% \caption{NP model comparison in LEAM simulator, population divided by 1000.}
% \begin{tabular}{c|c}
% \toprule
% Model & MAE \\
% % ====================== LA ======================
% \midrule
% NP \citep{garnelo2018neural} & 24.231 $\pm$ 5.884\\
%  \midrule
% SNP \citep{singh2019sequential} & 21.781 $\pm$ 0.825\\
%  \midrule
% STNP (Ours) & \textbf{6.291}$\pm$ 0.848\\
% \bottomrule
% \end{tabular}
% \label{tb:offline}
% \end{wraptable}

\paragraph{Ablation Study on NP Models.}
We perform ablation study on our proposed NP model, STNP. Compared with vanilla NP \citep{garnelo2018neural} and SNP \citep{singh2019sequential}, the key innovation of model is temporal latent process. To ensure fair comparison, we modified NP by adding the convolutional layers with diffusion convolution  \citep{li2018diffusion} to embed the graphs. Similarly, we modified SNP by replacing the convolutional layers with diffusion convolution. Figure \ref{fig:graphical_model} shows the corresponding graphical models. Table \ref{tb:offline} shows the testing MAE of different NP models trained in an offline fashion. Our STNP significantly improves the performance and can accurately learn the simulator dynamics.

\paragraph{Batch Active Learning with LIG.} 
\dwu{move to appendix}
In the case where we add more than one scenario of data per iteration,  LIG  allows us to calculate the corresponding reward for a batch of scenarios due to the mean aggregation layer in the NP encoder. In our LEAM-US experiment, we add $8$ scenarios per iteration (batch size $8$). As an ablation study, we  compared 4 different batch sizes, see  Appendix Figure \ref{fig:ablation_pred}. We observe that larger batch leads to better performance. This strategy combines LIG and random search, where it first randomly selects a set of groups and then use LIG to measure the reward for the data within each group. Random search encourages exploration whereas LIG  exploits the highest reward.


\subsection{Reaction-diffusion Simulator.}
\textbf{Reaction-diffusion Simulator.} 
The Reaction-diffusion Simulator is a spatial, temporal model to simulate how two chemicals might react to each other as they diffuse through a medium together. The simulation is based on the substances (initial pattern), feed rate, removal rate and reaction between two substances. Details of the model are deferred to the Appendix
\ref{}. \\

\textbf{Dataset.}
We use the simulator to generate sequences from 0 to 500 timestamps, sampled every 100 timestamps, resulting into 5 timestamps for each simulated sequence. Each sequence is simulated with a unique feed rate ($\theta_{0}$) and kill rate ($\theta_{1}$) combination. Overall, there are 200 scenarios in the search space, corresponding to 200 different $(\theta_{0}, \theta_{1})$ combinations. We split 80\% as the candidate train set and 20\% for validation and test.

\textbf{Model Implementation.}
We implement a STNP model to mimic the reaction diffusion simulator with feed rate ($\theta_0$) and kill rate ($\theta_1$) as input.We use the Convolution layers together with a linear layer to encode the spatial reaction data into latent space. We use an LSTM layer to encode the latent spatial data with $\theta_0$, $\theta_1$ to map the input-output pairs to hidden features. With $\theta_0$, $\theta_1$, the initial state of the reaction and a z sampled from the same posterior distribution, we use an LSTM layer and Deconvolution layers to simulate reaction diffusion sequence.

\textbf{STNP Predictions.}
Figure \ref{} left visualize the STNP predictions with same initial state, four different ($\theta_0$, $\theta_1$) and z sampled from a same posterior distribution. As the figure indicates each timestamp in the predictions of STNP matches the truth well. These results assure the STNP model's ability to serve as a deep surrogate model for the reaction diffusion simulator.

\textbf{Acquisition Functions.}
We compare different acquisition functions with STNP. All methods start
with the same 5 scenarios. Then we continue adding 5 scenarios to the training set until the validation loss converges. The test MAE is measured by averaging the performance over three random runs. Figure \ref{} right shows the log scale MAE versus the percentage of samples included during training. It shows our proposed LIG always has the best MAE performance until the convergence.

==> sections/preamble.tex <==
% \usepackage[dvipsnames]{xcolor}
% \newcommand{\M}[1]{{\mathbf{#1}}} % matrix
% \newcommand{\T}[1]{{\mathcal{#1}}} % tensor
% \newcommand{\V}[1]{{\mathbf{#1}}} % vector

% \usepackage[dvipsnames]{xcolor}
\newcommand*\ryu[1]{\textcolor{magenta}{[RY: #1]}}
\newcommand*\mc[1]{\textcolor{MidnightBlue}{[Matteo: #1]}}
\newcommand*\mya[1]{\textcolor{blue}{[Yian: #1]}}
\newcommand*\dwu[1]{\textcolor{red}{[Allen: #1]}}
\newcommand*\bn[1]{\textcolor{orange}{[Brooks: #1]}}


\newcommand*\lrb[1]{\left[#1\right]}
\newcommand*\lrbb[1]{\left\{#1\right\}}
\newcommand*\lrp[1]{\left(#1\right)}
\newcommand*\lrn[1]{\left\|#1\right\|}
\newcommand*\lrw[1]{\left\langle#1\right\rangle}
\newcommand{\rE}{{\mathbb E}}

\def\rT{{\rm T}}
\def\mI{\mathrm{I}}
\def\R{\mathbb{R}}
\def\A{A}
\def\E{e}
\def\mA{\mathrm{A}}

\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}

==> sections/unused.tex <==
\paragraph{Maximize the differential entropy} We can use entropy to quantify the amount of information given a new sample. By always selecting the sample with largest entropy, the system of samples will tend to obtain more information. In practice, it is hard to evaluate the differential entropy given continuous outputs. To alleviate this problem, we can apply Monte Carlo samples to estimate the differential entropy term $\mathbb{H}$.
By samples of $\hat{z}=\{z_1, ..., z_n\}$, we can obtain an empirical distribution of $\hat{x}|z, \mathcal{D}_{train}$. Further, via Kozachenko - Leonenko Estimate \cite{kraskov2004estimating} \mg{[need to figure out correct citations since papers don't have proper title]}, we can have
\begin{align}
    \mathbb{H}(x|z, \theta)&=-\int_c p(\hat{x}=c|z, \theta)\log p(\hat{x}=c|z, \theta)\\
    &\approx -\psi(k)+\psi(N)+\log c_d+\frac{d}{N}\sum_{i=1}^N \log\epsilon(i),
\end{align}
where $\psi(x)=\Gamma(x)^{-1}d\Gamma(x)/dx$ is the digamma function, $k$ is the nearest neighbour, $N$ is the number of sample, and $\epsilon(i)$ is twice the distance from $x|z_i, \theta$ to its k-th neighbour.
% By setting $r(x)=\log p(x|\theta^i)$, we can obtain an estimation of $\mathbb{H}(x|\theta^i)$ via the average of samples
% \begin{align*}
%     \mathbb{H}(x|\theta^i) &\approx \frac{1}{n}\sum\log p(\hat{x}_i|\theta^i)
% \end{align*}
% \[p(x|z, \theta^i)\]
% \[p(x|\theta^i)\]
% % action network (policy gradient)
% \[
% \log p(\hat{x}=c| \theta^{(i)}) \geq \Ep{q(z|\theta^{(i)})}{\log p(\hat{x}|z, \theta^{(i)})} - \text{KL}(q(z|\theta^{(i)})||p(z))
% \]
% \ry{Given a dataset $S$, can we train our neural process model sequentially and update the parameters?}

We can obtain an empirical distribution of $\hat{x}|\mathcal{S}$. 
At this point, we consider to add more samples to enlarge $\mathcal{S}_1$. We generate $m$ new uniform random samples $\{(\theta_{0:t}^1, x_{1:t}^1), ..., (\theta_{0:t}^m, x_{1:t}^m)\}$. In this way, we will have $m$ possible enlarged simulation data $\Tilde{\mathcal{S}}^i=\mathcal{S}\cup\{(\theta_{0:t}^i, x_{1:t}^i)\}$. 
With this enlarged simulation data, we hope to obtain the best enlarged simulation data sequentially using acquisition function. One way is to use the Mean STD to be the acquisition function. By generating $\mathbf{z}=\{z_1, z_2, ..., z_n\}$, one can estimate the Mean STD in the following: 
\begin{align*}
    \text{Mean STD}(\mathcal{S}^i) = \frac{1}{t}\sum_{s=1}^t\sigma(\mathcal{S}^i), \;\;\;\;\sigma^2(\mathcal{S}^i)=\frac{1}{|\mathbf{z}|-1}\sum_{j=1}^{|\mathbf{z}|} \left(\hat{x}_i-\frac{1}{|\mathbf{z}|}\sum_{j=1}^{|\mathbf{z}|}\hat{x}_i\right)^2,
\end{align*}
where $\hat{x}_i$ is obtained from $z_i$ given $\theta$ \mg{notation need to be unified}. 






\textbf{Remark}: when $\theta$ is time-varying, the optimization problem becomes more challenging. Here we start with a static $\theta$. So instead of solving for a sequence of values, we are solving for a few parameters.


$r(X,\theta)$ is the reward function at data $X$ when taking action $\theta$; Here $\theta$ can be thought of a set of parameters inside the simulator we wish to try 
